Mission Planning and Safety Assessment for Pipeline Inspection Using Autonomous Underwater Vehicles: A Framework based on Behavior Trees

The recent advance in autonomous underwater robotics facilitates autonomous inspection tasks of offshore infrastructure. However, current inspection missions rely on predefined plans created offline, hampering the flexibility and autonomy of the inspection vehicle and the mission's success in case of unexpected events. In this work, we address these challenges by proposing a framework encompassing the modeling and verification of mission plans through Behavior Trees (BTs). This framework leverages the modularity of BTs to model onboard reactive behaviors, thus enabling autonomous plan executions, and uses BehaVerify to verify the mission's safety. Moreover, as a use case of this framework, we present a novel AI-enabled algorithm that aims for efficient, autonomous pipeline camera data collection. In a simulated environment, we demonstrate the framework's application to our proposed pipeline inspection algorithm. Our framework marks a significant step forward in the field of autonomous underwater robotics, promising to enhance the safety and success of underwater missions in practical, real-world applications. https://github.com/remaro-network/pipe_inspection_mission

==> tex/04_simulation.tex <==
The generated behavior tree is integrated within a ROS-based simulation framework, as shown in Fig \ref{fig:GA}. The DUNE simulator is the runtime environment for vehicle onboard software that implements the simulation of the LAUV's mathematical model and allows the control of the simulated vehicle through IMC messages~\cite{LSTS-Toolchain}. 
The UNavSim simulator carries out the sensor simulation, including realistic renderings from the camera and segmentation annotations \cite{unavsim}. UNavSim and DUNE are synchronized through a ROS bridge that handles the communication between the two.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{img//simulation/unreal_screenshot.png}
    \includegraphics[width=0.5\linewidth]{img//simulation/neptus_screenshot.png}
    
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}

% The proposed simulated framework is deployed in an environment resembling the Porto Atlântico Marina to (1) demonstrate the proposed framework's safety and (2) record a simulated dataset aimed for sim-to-real transfer applications.  


